Fast End-to-End Wikification

Wikification of large corpora is beneficial for various NLP applications. Existing methods focus on quality performance rather than run-time, and are therefore non-feasible for large data. Here, we introduce RedW, a run-time oriented Wikification solution, based on Wikipedia redirects, that can Wikify massive corpora with competitive performance. We further propose an efficient method for estimating RedW confidence, opening the door for applying more demanding methods only on top of RedW lower-confidence results. Our experimental results support the validity of the proposed approach.

==> TW-EMNLP'19/PredictingRedWErrors.tex <==
\section{Identifying potential system errors}
\label{sec:RedWerrodDetection}
% ns We would like to rank RedW results by their risk to be errors, in order to determine the order by which the wikified terms will be sent for further analyses by heavier tools. To keep the system light-weight, it is essential that 
%%similarly to the Wikification process, 
%the ranking process will also be context-free and efficient.
Our next step is to provide an efficient method to properly estimate the confidence of RedW results, such that RedW errors will be characterized by low-confidence scores, which will be further Wikified by heavier tools.
To this end, we present a corresponding large-scale error-analysis of RedW results over Wikipedia.
% ns , based on which we suggest a method for scoring terms by their risk to be incorrectly Wikified.
% By 'incorrectly Wikified' we refer to two types of errors. 
There are two types of error:
i) linking a term to an incorrect page, while missing the correct page; ii) linking a term to a page while there is no Wikipedia page that corresponds to the meaning of the term in the sentence where it was spotted. 
We leverage Wikipedia internal links (WL) as ground truth against which we compare RedW results. % ns  of applying RedW %RA(or RedW+) 
% to the contents of all Wikipedia articles.
%RA (using the same Wikipedia dump enwiki-20180901 as was used to create the spotMap~\ref{sec:spotting})
%RA , statistically analyzing the agreement between the two. 
Given an article in which RedW resolves term $s$ to a Wikipedia page $C$, we assume that RedW is correct if the article contains a WL to $C$. The agreement between RedW and WL is defined on the article level since in Wikipedia
there is at most one WL per concept in an article, usually but not necessarily in the first time it is referred to. 
% ns* -- the following sentence is not that clear - perhaps rewrite?
Moreover, this definition reduces noise originating from the noisy nature of WLs, which sometimes associate the concept to neighboring terms instead of to the concept term itself. 
  
We treat articles where RedW detected a mention $s$ as independent Bernoulli variables, which take a value $1$ if RedW agrees with WL and $0$ otherwise.  
Let $N$ be the number of articles where RedW detects $s$ as a mention, and let $K$ be the number of articles among $N$ where RedW agrees with WL. The empirical probability of agreement between RedW and WL is $K/N$. We denote this probability by $SR$ (Success Rate). Notice that WLs provide only a partial coverage of the references to most concepts in Wikiepdia. An article can refer to a concept $C$ but have no WL to $C$, while in other cases the absence of WL is justified, namely the term does not refer to any concept. Thus, a disagreement between RedW and WL does not necessarily mean that RedW is incorrect. Since $SR$ measures the \textit{agreement} between RedW and WL, it underestimates the true probability for a correct answer by RedW.
Since all terms ``suffer" from the partial coverage of WLs, ranking the terms by $SR$ could have served our objective of sorting RedW results. However, different concepts have different levels of coverage by WLs, an effect that we would like to neutralize. % ns For this purpose, 
Thus, we normalize $SR$ by its highest value among all the terms that are mapped to the same concept by RedW.  We call this normalized score $SR_{norm}$. %RA (Normalized Success Rate). 
The assumption behind this normalization is that for most concepts, among all the terms which may refer to it, there is at least one term which does not have multiple senses. The $SR$ of this term is expected to suffer only from the partial coverage problem of that concept, thus normalizing all other terms of the concept by this value should neutralize this effect. 
In Section \ref{sec:experiments} we show that $SR_{norm}$ significantly outperforms other scores in predicting RedW/RedW+ errors.



==> TW-EMNLP'19/conclusions.tex <==
\section{Conclusions and future work}
\label{sec:conclusions}
We present a new, run-time oriented % ns friendly 
tool for context-free Wikification based on Wikipedia redirects, which allows to Wikify large corpora. Despite its simplicity, its performance is superior to other, heavier e2e systems on several datasets. We 
further show how to properly estimate the confidence of the system predictions,
% ns then suggest a method to compute a confidence score, $SR_{norm}$, for our system's annotations, 
%and show how it can be utilized for efficiently incorporating heavier Wikification methods on top of RedW. We 
and demonstrate the associated potential performance gain. 
The $SR_{norm}$ score can also be used to score entire documents (e.g., by averaging over all annotations in the document), 
%RA which is the desired resolution of texts when RedW is combined with heavy \textit{global} EL algorithms. 
% ns which is the desired resolution of texts to combine RedW with heavy \textit{global} EL algorithms. 
highlighting documents over which combining RedW with heavy \textit{global} EL algorithms would be most promising. 


==> TW-EMNLP'19/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Performance of RedW}
We first evaluate the performance of RedW compared to other e2e Wikification methods. Note, that RedW % ns is a high resolution Wikification tool which 
aims to Wikify % ns at wikifying 
all terms in a text which can be linked to a Wikipedia page, independent of their type and role. Thus entity linking datasets which focus either on NE ~\cite{AIDA,ACE-MSNBC} or on salient terms ~\cite{AQUAINT} are sub-optimal for this evaluation. 
We chose two comprehensive Wikification datasets for evaluation: Wiki-test and Trans-test (a dataset of spoken data) from ~\cite{YosiBenchmark}, and two datasets, IITB ~\cite{IITB} and Aquiant~\cite{AQUAINT}, that contain both named-entities and other entity types, but are not comprehensive as the former two. We compare RedW to two e2e widely used solutions: Tagme \cite{TAGME} and WAT \cite{WAT}\footnote{Using the best configuration for detecting all entity types}. 
Further, we employed GERBIL\footnote{http://gerbil.aksw.org/gerbil/} through which we also compared experimental results against AIDA~\cite{AIDA}, DBpedia Spotlight\footnote{https://www.dbpedia-spotlight.org/}~\cite{DBPediaSL}, 
and Babelfy~\cite{Babelfy}. % FREME and FOX~\cite{FOX}.
%RA - deleted this paragraph
%AIDA leverages the Stanford NER tagger to identify possible mentions, and the YAGO2~\cite{YAGO2} for knowledge base. It employs a combination of three local and global disambiguation algorithms.
%DBPedia Spotlight spots using a {\em surface form database}, constructed from a parsing of Wikipedia anchors, titles, redirects and disambiguation pages. It links entities through vector space modeling of the context of the mentions and the context of each candidate.
%Babelfy combines spotting and entity linking through a unified graph-based approach, using BabelNet~\cite{Babelnet} for its knowledge base, and a graph disambiguation algorithm that combines semantic signatures and sub-graph statistics of the candidate entities.
%Finally, RedW+ is a simple extension of RedW that solves disambiguation pages by selecting the Wikipedia page with the highest commoness (i.e., the page with the largest number of times that the n-gram was explicitly mapped to, in all Wikipedia) among all candidate pages that appear in the disambiguation page.  
%FREME and FOX emerged from a comprehensive evaluation of  
%15 different ensemble learning algorithms. 
Since IITB and Aquaint do not, in practice, include all mentions, we add IITB* and Aquaint* which are the result when using the method of evaluation described in \cite{EREL}, where an annotation is considered as false-positive if its term is matched or overlapped with a term of the benchmark, but the linked concept is different. Table \ref{tab:accuracy} shows that (1) RedW achieves the best F1 on all datasets except Aquaint*;
%RA (except for Aquaint* where TagME and WAT achieved better F1). 
(2) RedW, TagMe and WAT, which support all types of entities achieve high recall on all datasets, while the systems focusing on named entities only, achieve very low recall; (3) RedW achieves the highest precision on all datasets 
% ns (ranging from .67 to .82), 
while maintaining a relatively high recall; (4) RedW+ increases the recall at the cost of precision; % ns but suffers from lower precision than RedW. 
This is expected as disambiguation pages are more noisy and the simple commonness is a relatively naive solution. % ns too naive to handle them. 
We discuss in the next section what a heavier method could achieve on the hard mentions.    
%RA Note that IITB* is the results on IITB when using the method of evaluation described in \cite{EREL}, where an annotation is considered as false-positive if its mention is matched or overlapped with a mention of the benchmark, but the linked concept is different.

\begin{table*}[h!]
\small
	\begin{center}
    \small
		\begin{tabular}{l|c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|} 
			\cline{2-16}
			\multirow{2}{*}{} & 
				\multicolumn{3}{c||}{\textbf{IITB}} &
				\multicolumn{3}{c||}{\textbf{IITB*}} &
				\multicolumn{3}{c||}{\textbf{Trans}} &
				\multicolumn{3}{c||}{\textbf{Wiki}} &
				\multicolumn{3}{c||}{\textbf{Aquaint*}} \\
			\cline{2-16}
			 & P & R & F1  & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\ 
			 \hline
			 \multicolumn{1}{|l|}{TagMe} &
			  .12  & .48 & .19 & .65 & .48 & .55 & .33 & .51 & .41 & .42 & .58 & .49 & .81  & \textbf{.89} & \textbf{.85}\\
			\hline 
			 \multicolumn{1}{|l|}{WAT} &
			 .18 & .53 & .27 & .66 & .53 & .59 & .44 & .39 & .42 & .44 & .45 & .45 & .85 & .84 & .84 \\
            \hline 
             \multicolumn{1}{|l|}{AIDA} &
            \textbf{.51} & .16 & .20 & .62 &.15 & .19 & .05 & .01 & .02 & .27 & .08 & .14 & \textbf{.90} & .36 & .52  \\ 
            \hline 
             \multicolumn{1}{|l|}{SpotLight} & 
            .51 & .26 & .35  & .67 & .25 & .36 & .33 & .09 & .15 & .59 & .21 & .31 &  .82 & .46 & .59 \\ 
            \hline 
             \multicolumn{1}{|l|}{Babelfy} & 
           .22 & .17 & .18  & .41 & .17 & .20 & .03 & .01 & .02 & .22 & .07 & .12 & .76 & .36 & .50  \\ 
%            \hline 
%            FREME & 
%             0.11 & 0.1 & 0.02  & 0.08 & 0.34 \\ 
%            \hline 
%            FOX & 
%             0.19 & 0.18 &  & 0.13 & 0.44  \\ 
            \hline
			\multicolumn{1}{|l|}{RedW} &
			 .26 & .67 & \textbf{.37} & .78 & .69 & .73 & \textbf{.76} & .62 & \textbf{.68} & \textbf{.72} & .64 & \textbf{.68} & .86 & .78 & .82 \\
            \hline 
			\multicolumn{1}{|l|}{RedW+} & 
			.19 & \textbf{.69} & .30 & \textbf{.80} & \textbf{.69} & \textbf{.74} & .57 & \textbf{.64} & .60 & .57 & \textbf{.67} & .62 & .83 & .79 & .81 \\
			\hline
		\end{tabular}
		\caption{\small Comparison of e2e methods - $Precision, Recall, F1$.}
         \label{tab:accuracy}       
       \end{center}
       \label{RedWResults}
\end{table*}

\subsection{Runtime performance}
%RA As mentioned above, the runtime of RedW is quite fast. 
Table~\ref{tab:runtime} reports runtime of RedW and TagMe on short text snippets of size 100-600 characters, as well as on a large news corpus of size 600Gb.   
The experiments were done on a single Linux-based computer comprising 14 processors in each of 2 cores and a total memory of 60 Gb.
%RAAs can be seen, 
RedW runtime is improved by more than an order of magnitude compared to TagMe.
% ns The runtime of RedW is 10-20 times faster than that of TagMe.

\begin{table}[tbh]
\small
	\begin{center}
    \small
		\begin{tabular}{|l|c|c|} 
		    \hline 
		        & Short snippets &  Large corpus \\
			\hline
			 TagMe & 113.96 ms & 22 days \\
			\hline
			  RedW & 5.3 ms & 41 hours \\
			\hline  
		\end{tabular}
		\caption{\small Runtime performance}
         \label{tab:runtime}       
       \end{center}
\end{table}

%RA \subsection{Confidence score for our system results}
\subsection{Confidence score}
%RA As was mentioned before, one can improve performance over RedW results by applying a heavier context-dependent D2W/pruning methods to a subset of the corpus, where the size of the subset depends on the run-time constraints.
%RA We compare between several methods for ranking RedW results. All methods are based on scoring the terms, ranking them according to their score, and selecting the top ranked terms as a subset for further processing. The difference between the methods is the score used for ranking. 
We compare $SR_{norm}$ (see Section \ref{sec:RedWerrodDetection}) to several baselines: (1) $rand$ -- the trivial random score; (2) $f_{max}$ -- the frequency of $C$ among concepts that $s$ is linked to, computed based on WLs population; (3) ${in}_{links}$ -- the number of incoming WLs to $C$. Note that ${in}_{links}$ assigns the same score to all the terms that are linked to $C$ by RedW; (4) $SR$ -- to examine the effectiveness of the intra-concept normalization performed in $SR_{norm}$.
Clearly, the potential precision gain from applying heavy Wikification methods increases with the error rate within the subset on which they are applied. We therefore evaluate the methods on the task of detecting errors by RedW+, which provides higher recall and lower precision compared to RedW. 
% ns Since RedW+ has higher recall but lower precision than RedW,
%RA (it spots and solves also the 'may refer to' terms which are prone to disambiguation errors)
% the effectiveness of the score in terms of precision and F1 improvements, is higher for the RedW+ version. 
Figure \ref{fig:RedErrors} shows precision-recall curves for the task of detecting RedW+ errors, when different scoring methods are used to rank the elements in the Wiki-test dataset. Clearly, $SR_{norm}$ significantly outperforms all other scores. 
%RA $SR$ is inferior to $SR_{norm}$ indicating that the inner-concept normalization is effective. $SR$ yields the best results across all datasets for both RedW and RedW+ (see supplementary material).  
\begin{figure}[ht!]
\centering
\includegraphics[width=75mm]{fig1_RedW+.png}
%RA\caption{Precision (fraction of RedW+ errors within the subset) vs. Recall (fraction of detected RedW+ errors) for several scoring methods on Trans-test. \label{fig:RedErrors}}
\caption{\small Precision (fraction of errors in the subset) vs. Recall (fraction of detected errors) on Trans-test. 
\label{fig:RedErrors}}
\end{figure}

%RANext we examine the potential performance improvement as a result of using $SR_{norm}$ for selecting the subset of texts to be processed by heavy methods. 
Next we examine the potential performance gain of using $SR_{norm}$ for selecting the subset of texts to be processed by heavy methods. To this end we assume an ideal method, able to correct all the disambiguation errors of the system and prune all terms mistakenly detected as mentions. Figure~\ref{fig:improvement} shows the ratio of improvement in the precision of RedW+, when the subset is selected by $SR_{norm}$, 
%RAcompared to the values obtained by selecting the subset at random. 
compared to selecting at random. 
%RAFor example, %RAon the Wiki dataset, the improvement when selecting $20\%$ of the mentions is $~12\%$.  
The results demonstrate the potential effectiveness of the $SR_{norm}$ scoring method. The maximal gain exceeds $10\%$ in all datasets. In the region of interest (small subsets), the improvement increases monotonically.
%MOVE TO APPENDIX
\begin{figure}[ht!]
\centering
\includegraphics[width=65mm]{Precision+.png}
\caption{Ratio between precision obtained by an ideal system as a result of selecting the subset using $SR_{norm}$ and a random selection of the subset.  \label{fig:improvement}}
\end{figure}

%Finally, a simple and low cost usage of $p_{norm}$ is for precision improvement, using aggressive pruning. For example in IITB, pruning $10\%$ of the RedW annotations using the top ranked annotations  
  




==> TW-EMNLP'19/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
The two key challenges faced by end-to-end (e2e) Wikification systems are \textit{Spotting}, i.e. identifying the terms in a text\footnote{A term can be one or more tokens} that should be Wikified, and \textit{Entity Linking (EL) to Wikipedia}, identifying the relevant Wikipedia page among a set of candidate pages. The latter task is usually more runtime demanding, due to the need to consider the context of the mention when aiming to select the most relevant page. 

%Existing end-to-end Wikification methods (REF TagMe, WAT(REF) Wikify) are 
Existing e2e Wikification methods \cite{TAGME, WAT,wikify} are 
%RA performance oriented, namely their emphasis is put on
%RA
focused on achieving maximal precision and/or recall, while run time is considered a secondary issue. % ns
However, many NLP tasks, such as argumentation mining \citep{W17-5110}
% ns , coreference resolution \citep{RatinovRo12} 
and question answering \citep{conf/emnlp/BerantCFL13} 
% ym P15-1128}, 
can % ms substantially 
benefit from Wikifying large corpora, marking the need for light-weight solution.
% ns which requires a light-weight Wikification system with low computational demands. 

%RA For this purpose we suggest a run-time oriented approach for Wikification, which combines two layers: a light-weight end-to-end context-free wikification layer (CFL), which solves both the MD and the D2W problems, and a more precise but heavier context-dependent D2W layer (CDL). The CFL enables to Wikify large corpora in minimal run-times but sub-optimal precision, while the heavier and more accurate CDL increases performance by being applied to a subset of texts in the corpus. , where the subset’s size depends on the run-time requirements, and serves as a dial that can be tuned to the desired point in the run-time - performance space.

%RA - rewrote above paragraph
%For this purpose we suggest a run-time oriented approach for Wikification, which combines two layers. First, a light-weight end-to-end context-free wikification layer, which solves both the MD and the D2W problems in minimal run-time with a high, even if sub-optimal, precision. Second, a more precise but heavier context-dependent D2W layer (CDL), which is applied to a subset of texts in the corpus, based on the confidence of the first layer. The user can adjust the size of this subset depending on the run-time requirements. This combined approach enables tuning to a desired point in the run-time - precision space. %RA note that performance is also often referring to runtime so better use precision or accuracy

%RA - rewrote it again
%RA For this purpose we suggest a run-time oriented approach for Wikification. 
Here, we present RedW\footnote{A demo is available at \href{http://bit.ly/redwe2e}{http://bit.ly/redwe2e}}, a highly efficient e2e context-free wikification layer
% ns , which solves both the Spotting and  EL problems in minimal run-time with 
%a high, even if sub-optimal, 
with competitive precision, % by harnessing 
that relies on the wisdom of the crowd as reflected through ``redirect'' pages of Wikipedia\footnote{\href{https://en.wikipedia.org/wiki/Wikipedia:Redirect}{https://en.wikipedia.org/wiki/Wikipedia:Redirect}}. 
% ns
Using this method, we were able to Wikify a corpus of nearly 10 billion sentences with satisfactory precision, providing highly valuable results for various downstream NLP applications.\footnote{To keep the anonymity of this submission, more details will be shared in the final version.}
%RA 
%Unlike many existing methods, it aims
%RA
%RA aiming 
RedW aims to wikify as many mentions as possible, not only named entities \cite{AIDA,ACE-MSNBC} or salient terms \cite{ERD'14,AQUAINT}. 
%We adopt a complete approach of Wikification, 
%RA
%which is useful for several downstream NLP tasks, 
%This is useful for several downstream NLP tasks such as QA and argument mining. 
% ns The method enabled to fully wikify a corpus of 10 billions sentences that could not have been wikified by other systems due to unfeasible run-times.
%RA One key challenge in this setting is developing a light-weight Wikification system with high performance and short run-times. We propose RedW, a simple and efficient end-to-end Wikification method which harnesses the wisdom of the crowd through "redirect" pages of Wikipedia (https://en.wikipedia.org/wiki/Wikipedia:Redirect). 
%RA - deleted this paragraph. moved a few points above
%RedW 
%is a simple and efficient e2e Wikification method which 
%harnesses the wisdom of the crowd through "redirect" pages of Wikipedia\footnote{\href{https://en.wikipedia.org/wiki/Wikipedia:Redirect}{https://en.wikipedia.org/wiki/Wikipedia:Redirect}}.
%The redirects are used to solve both the Spotting and the EL problems in a quick and context-independent way. This method provides scalable Wikification of large corpora with minimal run times and competitive accuracy. The method enabled to fully wikify a corpus of 10 billions of sentences that could not have been wikified by other systems due to unfeasible run-times.
%only a subset of the terms in a document. Some studies focus on wikifying 
%RA Another key challenge of the suggested approach is selecting the corpus subset to be processed by the heavy CDL in a way which will optimize the potential precision gain of the entire system. The way this subset is selected can have a dramatic influence on the overall performance. Obviously, the aim is to apply this time-consuming layer to those texts which need it most, i.e. textual regions in the corpus where the D2W of RedW performs poorly.  
We further present an efficient method for scoring RedW results, allowing a user to identify a subset of terms over which to apply heavier, more precision oriented methods. We demonstrate that the potential performance gain from using this method is substantial. This combined approach enables tuning to a desired point in the run-time - precision space. 

%RA A key to the success of the proposed approach is selecting the corpus subset for the heavy-weight analysis, in a way which optimizes the potential precision gain of the entire system. 
%RA The way this subset is selected can have a dramatic influence on the overall performance. 
%Obviously, the aim is to apply any time-consuming methods to those texts which need it most, i.e. textual regions in the corpus where RedW performs poorly. We suggest a method for scoring terms by their risk to be erroneously wikified by RedW, and demonstrate its effectiveness by showing that the potential performance gain from using this method is substantial. 

%RA To this end, 
%RA Further, we suggest several methods for identifying the ‘weak regions’ of the corpus, by scoring terms based on their risk to be linked to an incorrect Wikipedia page by RedW. We evaluate these methods using several Wikification datasets, and show that ranking the terms by NBPCI, a score we designed which is based on Binomial Proportion Confidence Interval, yields the best results. We further demonstrate that the potential gain from identifying the weak regions is substantial. We publish a resource with all Wikipedia redirects and their NBPCI score for future research.




 

  



==> TW-EMNLP'19/related.tex <==
\section{Related work}
\label{sec:related}
A straightforward approach to context-free EL is selecting the most likely Wikipedia title of a given term, based on anchor dictionaries such as cross-wikis \citep{L12-1109}. This has been shown to be a strong baseline for EL \citep{chang, ACE-MSNBC,Fader09scalingwikipedia-based}. Here, instead of relying on static dictionaries generated from crawling the web \citep{L12-1109} or by aggregating anchor links in Wikipedia, we leverage the dynamic and powerful machinery of Wikipedia redirects.
%RA to create an efficient and competitive context-free Wikification system. 
Redirects have been incorporated before in e2e Wikification systems as part of the Spotting step \citep{TAGME, WAT, wikify}. 
% ns However, in RedW, redirects are used to solve both the Spotting and the EL tasks.  To the best of our knowledge, RedW is the first context-free e2e Wikification system.
However, RedW uses redirects to further solve the EL task; hence, to the best of our knowledge, it is the first context-free e2e Wikification system, 

% ns - edited
Existing e2e Wikification methods ~\cite{WAT,TAGME} use context dependent EL algorithms, and thus focus on performance rather than runtime. 
% aiming to optimize performance, while run-time considerations are usually left out-of-scope. 
Moreover, the computational requirements of EL methods have increased dramatically %RA throughout the past years, 
with the flourishing of neural models,  \citep{conf/acl/HeLLZZW13,DBLP:journals/corr/YamadaS0T16,DBLP:journals/corr/GaneaH17,Sun:2015:MMC:2832415.2832435}
which have established state-of-the-art performance results, while further increasing computational demands.
 %RA with respect to performance, 
%  but at the same time increased computational demands.
% ns
% In contrast, 
%RA we tackle the Wikification problem from a runtime-friendly viewpoint. Motivated 
% motivated by the benefits of being able to Wikify large corpora, we suggest a method for obtaining high quality Wikification results in short run-times.

% ns Among the works which did consider run-time as a main issue, 
In contrast, \cite{nguyen2014aida} % ns uses a novel 
consider an efficient two-stage mapping algorithm. It first identifies a set of “easy” mentions with low ambiguity and links them to entities in a highly efficient manner. Next, it harnesses the high-confidence linkage of “easy” mentions to establish more reliable contexts % ns for  disambiguation of 
to disambiguate the remaining mentions.
However, this work focuses only on the NER problem, rather than on the full problem of spotting and linking. 
Another run-time oriented work is \cite{hogan2012scalable}; 
% ns , but the problem they study is different, namely 
there, the authors focus on consolidating entity linking datasets by inter-linking the individual datasets (finding links between equivalent entities) rather than spotting and linking a corpus from scratch. 

%
%Disambig without context is expected to yield better results when relying on linking data derived from context-free text strings.
%the disctionaries are based on Strings with context. redirect is based on statisctics derived from the text strings only.
%These disctionaries include a lot of noise (ref) and do not include links to disambiguation pages.
%redirects have less noise since strings with poor statistics are not included in the redirect list, and inconclusive strings are directed to disambig pages. 
%redirects have some advantages over these disctionaries. they use the wisdom of crowd in solving disambiguation

==> TW-EMNLP'19/termWikifier.tex <==
\section{RedW: A Redirect-Based Wikification}
\label{sec:termWikifier}
%RA We tackle the e2e Wikification task, namely: 
The e2e Wikification task consists of (1) \textbf{Spotting} -- detecting terms that are candidates to become mentions; (2) \textbf{Entity Linking} -- discard (prune) candidate terms or link them to Wikipedia entities. 
%RA The basic idea behind RedW is that in many cases, a term as is, or up to some simple editorial transformations, matches a title, or matches a \textit{redirect} page that leads to the default, most frequently used sense thereof, which is expressed as a title of a Wikipedia page.  
% ns The basic observation behind RedW is that in many cases, 
RedW relies on the assumption that a term - up to some simple editorial transformations - often matches its Wikipedia title, or a corresponding  Wikipedia \textit{redirect} page.
% ns that leads to the default, most frequently used sense of the term, which is a Wikipedia title.
%RA Our basic idea is to harness the wisdom of the crowd through "redirect" pages of Wikipedia, to find the terms to be Wikified, and link them to the appropriate Wikipedia article.
% ns We thus 
Thus, RedW harnesses the wisdom of the crowd as expressed in ``redirect'' pages, to find the terms to be Wikified, and link them to the appropriate Wikipedia article.
%le
A main advantage of using redirects over anchor dictionaries ~\cite{L12-1109} is their dynamic nature. They are maintained and updated both automatically and by Wikipedia editors \cite{hill2014consider}, hence are expected to contain less noise compared to 
% ns The human involvement, which includes review and removal of redirects, results in reduced noise compared to 
automatically created dictionaries. 
% ns The subsequent sub-sections describe the Spotting and EL in more details.
%%%
%RedW checks whether there is a matching Wikipedia page, that is not a disambiguation page\footnote{A page is a disambiguation page if it has the text: \textit{may also refer to} in its first sentence}.   
%Our hypothesis is that having two evidences - both a term and a matching title - increase the likelihood that this is a correct mention. 
 
%Finally, we present a version (abbreviated \textit{TWDP}) that prunes some already resolved mentions. The method requires just the term, the resolved wikipedia title and the surrounding sentence, and we show its efficiency compared to other methods. 

%In the following sub-sections we describe the spotting of the RedW and the above three versions.

\subsection{Spotting}
\label{sec:spotting}
We pre-process Wikipedia\footnote{We use the dump enwiki-20180901 from Sep 2018} and build \textit{spotMap} -- a table of all Wikipedia titles, including the redirect titles. 
%RA We refer to it as \textit{spotMap}. 
% ns \textit{SpotMap} contains both real titles as well as redirect titles.  
%The redirect titles are mapping from a source title to a target title. They contain different forms of the 
%liat% to check with yosi
%direct
%%
%title, including some transformations (e.g., plurals) and potential spelling errors. 
%In addition to the spotMap we keep also a table of titles that we do not want to solve (such as movies, journals, etc). We refer to it as \textit{blackList}.
Given a new text, we try to match its n-grams to \textit{spotMap}, preferring  longer matches. Thus, we start with $n=10$, and gradually move to smaller $n$'s. 
%For each n-gram, we capitalize its first letter (to conform to the Wikipedia titles format) and check whether it appears in \textit{spotMap}. 
Per n-gram, we check whether it appears in \textit{spotMap}, after capitalizing its first letter. % ns to conform with Wikipedia  format. 
%Matched n-grams serve for two purposes. First, they are kept as candidate mentions for the next step. Second, their tokens are marked so that they will not participate in other candidate n-grams (to avoid noisy short n-grams that are included in or overlap with longer titles). The final list of matched n-grams are passed to the EL step.
Matched n-grams are kept as candidate mentions for the next step. Further, their tokens are marked to avoid including them in subsequent -- shorter -- candidate n-grams. 
% ns so that they will not participate in other candidate n-grams (to avoid noisy short n-grams that are included in or overlap with longer titles). 
The final list of matched n-grams is analyzed by % ns is passed to 
the EL step.

\subsection{Entity Linking}
\label{sec:base-TW}
Given a candidate term and its matched title/redirect, % ns ) from the spotting step, we try to resolve it to a mention (namely, link it to a Wikipedia page). 
RedW aims to link it to the corresponding Wikipedia page, unless
%We first apply simple pruning rules which filter out terms that are stop words or that start with one of the prepositions \{in, at, on, of, by, is\}. 
% If the term corresponds to a redirect, the target title is selected. 
% If 
the resulting page is a disambiguation page
%RA\footnote{A page is a disambiguation page if it has the text: \textit{may [also] refer to} in its first sentence}
\footnote{I.e., has the text \textit{may [also] refer to} in its first sentence}.
% ns we discard the term. Otherwise, we link the term to the above resulting title. 
Our hypothesis is that having two evidences - both a term and a matching title/redirect - increases the likelihood that this is a correct mention.
Discarding terms corresponding to disambiguation pages reduces recall. 
We therefore propose % ns a variant of RedW, denoted 
RedW+, which when given a term and a matching disambiguation page, links the term to its most common page among all pages pointed from the disambiguation page. 
% ym which links such terms to the page with the maximal Wikipedia in-degree, i.e., % ns corresponding to their 
%the most frequent meaning. 
Clearly, the increase in recall comes at the expense of precision. As mitigation, we demonstrate how our suggested confidence score can be used to increase precision.

%
%We can further embed the TW in a full Mention detection tool as follows. Given a text, take all n-grams as candidate Spots.  Then disambiguate each spot using the TW.  

%We deal with the problem of disambiguating a given term (consisting of one or more tokens) to its most appropriate sense in a Knowledge Base (abbreviated KB) such as Wikipedia. 




